Scatter correction based on quasi-Monte Carlo for CT reconstruction

Scatter signals can degrade the contrast and resolution of computed tomography (CT) images and induce artifacts. How to effectively correct scatter signals in CT has always been a focal point of research for researchers. This work presents a new framework for eliminating scatter artifacts in CT. In the framework, the interaction between photons and matter is characterized as a Markov process, and the calculation of the scatter signal intensity in CT is transformed into the computation of a $4n$-dimensional integral, where $n$ is the highest scatter order. Given the low-frequency characteristics of scatter signals in CT, this paper uses the quasi-Monte Carlo (QMC) method combined with forced fixed detection and down sampling to compute the integral. In the reconstruction process, the impact of scatter signals on the X-ray energy spectrum is considered. A scatter-corrected spectrum estimation method is proposed and applied to estimate the X-ray energy spectrum. Based on the Feldkamp-Davis-Kress (FDK) algorithm, a multi-module coupled reconstruction method, referred to as FDK-QMC-BM4D, has been developed to simultaneously eliminate scatter artifacts, beam hardening artifacts, and noise in CT imaging. Finally, the effectiveness of the FDK-QMC-BM4D method is validated in the Shepp-Logan phantom and head. Compared to the widely recognized Monte Carlo method, which is the most accurate method by now for estimating and correcting scatter signals in CT, the FDK-QMC-BM4D method improves the running speed by approximately $102$ times while ensuring accuracy. By integrating the mechanism of FDK-QMC-BM4D, this study offers a novel approach to addressing artifacts in clinical CT.

==> README <==
# harvard family of bibliographic styles
# Copyright 1994 - Peter Williams pwil3058@bigpond.net.au
#
# This work may be distributed and/or modified under the
# conditions of the LaTeX Project Public License, either version 1.3
# of this license or (at your option) any later version.
# The latest version of this license is in
#   http://www.latex-project.org/lppl.txt
# and version 1.3 or later is part of all distributions of LaTeX
# version 2005/12/01 or later.
#
# This work has the LPPL maintenance status `maintained'.
# 
# The Current Maintainers of this work are Peter Williams and Thorsten Schnier.
#
# This work consists of all files listed in manifest.txt.
#
# Licence notice added on behalf of Peter Williams and Thorsten Schnier
# by Clea F. Rees 2009/01/30.

This is version 2.0.5 of the harvard family of bibliographic styles.
It is a bug fix of 2.0 which was a major rewrite to bring the sty file into
line with the new latex described in ``The LaTeX Companion''.  Due to the
efforts of Thorsten Schnier (thorsten@archsci.arch.su.edu.au) it incorporates
support for the LaTeX to html translator by Nikos Drakos
(nikos@cbl.leeds.ac.uk).

It includes a fixes by Berwin A. Turlach (berwin@alphasun.anu.edu.au) for
problems with \AtBeginDocument introduced in the latest version of LaTeX2e
and problems with the \nocite command.

A new style apsr.bst (American Political Science Review) is enclosed
courtesy of Nathaneil L. Beck (nbeck@weber.ucsd.edu)

NB.  The file harvard.sty makes considerable use of features in the new latex
that were not present in latex version 2.09 and is, therefore, not compatible
with that version.  However, the *.bbl files produced by the various bst files
should be still useable with latex version 2.09.

The following files are enclosed.

  README	- This file
  INSTALL	- Installation instructions
  Makefile	- Makefile for installation
  harvard.ps	- Postscript version of the documentation
  harvard.tex	- LaTeX source for the documentation
  harvard.bib	- BibTeX database file for the documentation
  doc_Makefile	- Makefile for documentation
  harvard.sty	- LaTeX style file for harvard bibliographic style
  harvard.perl	- LaTeX2html style file for harvard bibliographic style
  agsm.bst	- harvard BibTeX style file to satisfy the requirements
		  of the Australian Government Style Manual
  dcu.bst	- harvard BibTeX style file to satisfy the requirements
		  of the Design Computing Unit, Sydney University
  <other>.bst	- various style files contributed by users

Online documentation is available via the WWW at:

HREF="http://www.arch.su.edu.au/~peterw/latex/harvard/"

